Sampling-Based Estimates of the Sizes of Constrained Subcodes of Reed-Muller Codes

This paper develops an algorithmic approach for obtaining approximate, numerical estimates of the sizes of subcodes of Reed-Muller (RM) codes, all of the codewords in which satisfy a given constraint. Our algorithm is based on a statistical physics technique for estimating the partition functions of spin systems, which in turn makes use of a sampler that produces RM codewords according to a Gibbs distribution. The Gibbs distribution is designed so that it is biased towards codewords that respect the constraint. We apply our method to approximately compute the sizes of runlength limited (RLL) subcodes and obtain estimates of the weight distribution of moderate-blocklength RM codes. We observe that the estimates returned by our method are close to the true sizes when these sizes are either known or computable by brute-force search; in other cases, our computations provide provably robust estimates. As an illustration of our methods, we provide estimates of the weight distribution of the RM$(9,4)$ code.

==> wtdist.tex <==
In Section \ref{sec:estimate}, we discussed a technique to obtain estimates of the sizes of (potentially arbitrarily-)constrained subcodes of RM codes. In this section, we restrict our attention to the constant weight constraint; in other words, we shall concern ourselves in this section to exact computation of the weight distribution of RM codes, algorithmically. While our interest is primarily on RM codes, our exposition here applies to arbitrary linear codes that are constructed using the Plotkin $(\mathbf{u} , \mathbf{u}+\mathbf{v})$ construction.

Consider a pair $\cC_0 \subseteq \cC$ of nested linear codes over $\F_2$ \footnote{The results in this section are applicable for any field $\F_q$.} (observe that the RM family of codes obeys such a nesting property; in particular, RM$(m,r-1)\subseteq \text{RM}(m,r)$, for $m\geq 1$ and $1\leq r\leq m$). Let  $\cC_0, \cC_1,\ldots,\cC_{M-1}$ be an enumeration of the cosets of $\cC_0$ in $\cC$, where $M = |\cC/\cC_0| = 2^{\dim\cC - \dim \cC_0}$. 

Let $A_{\cC}(z)$ and $A_{\cC_i}(z)$ denote the weight enumerator polynomials of $\cC$ and $\cC_i$, respectively. Since $\cC$ is the disjoint union of the $\cC_i$s, we have
$$
A_{\cC}(z) = \sum_{i=0}^{M-1} A_{\cC_i}(z).
$$

Let $\overline{\cC}$ be the code obtained from $\cC$ and $\cC_0$ using the $(\u , \u+\v)$ construction:
$$
\overline{\cC} = \{(\u,\u+\v) : \u \in \cC, \v \in \cC_0\}.
$$

\begin{lemma}
	\label{lem:1}
	The weight enumerator of $\overline{\cC}$ is given by
	$$
	A_{\overline{\cC}}(z) = \sum_{i=0}^{M-1} {(A_{\cC_i}(z))}^2.
	$$
\end{lemma}
\begin{proof}
	We only need the observation that for any $\u \in \cC$ and $\v \in \cC_0$, $\u$ and $\u+\v$ belong to the same coset $\cC_i$. 
	Thus,
	\begin{align*}
		A_{\overline{\cC}}(z) &= \sum_{\u \in \cC} \sum_{\v \in \cC_0} z^{w_H(\u,\u+\v)} \\
		&= \sum_{i=0}^{M-1} \sum_{\u \in \cC_i} \sum_{\v \in \cC_0} z^{w_H(\u)} z^{w_H(\u+\v)} \\
		&= \sum_{i=0}^{M-1} \sum_{\u \in \cC_i} z^{w_H(\u)} \sum_{\mathbf{v'} \in \cC_i} z^{w_H(\mathbf{v'})} \\
		&= \sum_{i=0}^{M-1} A_{\cC_i}(z) \cdot A_{\cC_i}(z).
	\end{align*}
\end{proof}

In the case of Reed-Muller codes, we have a situation such as the following: there is a nested sequence of codes $\cC_{00} \subset \cC_0 \subset \cC$, and another nested pair $\overline{\cC}_0 \subset \overline{\cC}$ such that $\overline{\cC}_0$ (resp. $\overline{\cC}$) is obtained from $\cC_{00}$ and $\cC_0$ (resp.\ $\cC_0$ and $\cC$) via the $(u \mid u+v)$ construction:
$$
\overline{\cC}_0 = \{(u,u+v) : u \in \cC_0, v \in \cC_{00}\}  \ \ \text{ and } \ \  \overline{\cC} = \{(u,u+v) : u \in \cC, v \in \cC_0\}.
$$
In this terminology, $\cC_{00}, \cC_0,$ and $\cC$ can respectively be associated with RM$(m,r-2)$, RM$(m,r-1)$ and RM$(m,r)$, and then $\overline{\cC}_0 = \text{RM}(m+1,r-1)$ and $\overline{\cC} = \text{RM}(m+1,r)$, where $m\geq 1$ and $2\leq r\leq m$.
We show below that the weight enumerator polynomial of a coset of $\overline{\cC}_0$ in $\overline{\cC}$ is computable from the weight enumerators of the cosets of $\cC_{00}$ in $\cC$.

We introduce some convenient notation first. Let $M$ and $M_0$ be the size of the quotient spaces $\cC/\cC_0$ and $\cC_0/\cC_{00}$, respectively, so that $M \cdot M_0$ is the size of $\cC / \cC_{00}$. Enumerate the cosets of $\cC_0$ in $\cC$ as $\cC_0, \cC_1, \ldots, \cC_{M-1}$, and those of $\cC_{00}$ in $\cC_0$ as $\cC_{00}, \cC_{01}, \ldots, \cC_{0,M_0-1}$. We extend this to a listing, $\cC_{ij}$, $i = 0,1,\ldots,M-1$, $j = 0,1,\ldots,M_0-1$, of the cosets of $\cC_{00}$ in $\cC$ as follows: if $\cC_i = \mathbf{u'} + \cC_0$ and $\cC_{0j} = \mathbf{v'} + \cC_{00}$ for some $\mathbf{u'} \in \cC$ and $\mathbf{v'} \in \cC_0$, then $\cC_{ij} = \mathbf{u'}+\mathbf{v'}+\cC_{00}$. With this, we have $\cC_{ij} \subset \cC_i$ for all $i,j$. Recall that $\cC/\cC_0$ and $\cC_0/\cC_{00}$ are $\F_q$-vector spaces. The induced vector space structure on $\cC / \cC_{00}$ is such that for all $\a, \b \in \F_q$, we have $\a \cdot \cC_{ij} + \b \cdot \cC_{kl} = \cC_{st}$ iff $\a \cdot \cC_i + \b \cdot \cC_k = \cC_s$ and $\a \cdot \cC_{0j} + \b \cdot \cC_{0l} = \cC_{0t}$.

As usual, let $A_{\cC_i}(z)$ and $A_{\cC_{ij}}(z)$ denote the weight enumerators of $\cC_i$ and $\cC_{ij}$, respectively.
\begin{lemma}
	\label{lem:2}
	Let $\u \in \cC$ and $\v \in \cC_0$ be given, so that $(\u,\u+\v) \in \overline{\cC}$ and $[\u,\u+\v]  := (\u,\u+\v) + \overline{\cC}_0$ is a coset of $\overline{\cC}_0$ in $\overline{\cC}$. Let $\cC_i := \u + \cC_0$ and $\cC_{0j} = \v + \cC_{00}$. Then, the weight enumerator of $[\u,\u+\v]$ is given by
	$$
	A_{[\u,\u+\v]}(z)  \ = \ \sum_{l=0}^{M_0-1} A_{\cC_{il}}(z) \cdot A_{\cC_{il} + \cC_{0j}}(z) 
	$$
\end{lemma}
\begin{proof}
	Observe that the set $\cC_i$ is the union of all the disjoint sets $\cC_{il}$ where $0\leq l\le M_0 -1 $.
	Thus,
	\begin{align*}
		A_{[u,u+v]}(z) &= \sum_{\c \in \cC_0} \sum_{\mathbf{c'} \in \cC_{00}} z^{w_H(\u+\c,\u+\v+\c+\mathbf{c'})} \\
		&= \sum_{l=0}^{M_0-1} \sum_{\mathbf{c''} \in \cC_{il}} \sum_{\mathbf{c'} \in \cC_{00}} z^{w_H(\mathbf{c''})} z^{w_H(\mathbf{c''}+\v+\mathbf{c'})} \\
		&= \sum_{l=0}^{M_0-1} \sum_{\u \in \cC_{il}} z^{w_H(\mathbf{c''})} \sum_{\x \in \cC_{il} + \cC_{0j}} z^{w_H(\x)} \\
		&= \sum_{l=0}^{M_0-1} A_{\cC_{il}}(z) \cdot A_{\cC_{il} + \cC_{0j}}(z)
	\end{align*}
\end{proof}
\section{Simplifying Computations Using the Automorphism Group}
Consider now the computation of weight distributions of binary Reed-Muller (RM) codes. First, for some preliminaries. Recall that RM codes of blocklength $2^m$ consist of the evaluations of multilinear polynomials $f\in \mathbb{F}_2[x_1,\ldots,x_m]$ over vertices of the $m$-dimensional unit hypercube. In particular, the $r^{\text{th}}$-order binary RM code RM$(m,r)$ can be written as
\[
\text{RM}(m,r) = \{\text{Eval}(f): f\in \mathbb{F}_2[x_1,\ldots,x_m] \text{ and deg}(f)\leq r \},
\]
where we use the notation Eval$(f):= \left(f({y}): {y} = (y_1,\ldots,y_m) \in \{0,1\}^m\right)$, with the coordinates ${y} = (y_1,\ldots,y_m)$ being ordered according to the standard lexicographic ordering. Moreover, given $f\in \mathbb{F}_2[x_1,\ldots,x_m]$, we define deg$(f)$ to be the largest degree of a monomial present in $f$. 

From the definition above, the following facts can be deduced (see Chapter 13 of \cite{mws}): the dimension dim$(\text{RM}(m,r)) = {m\choose [0:r]}$, where we use the notation ${n\choose [a:b]}$ to mean $\sum_{i=a}^{b} {n\choose i}$, for $a\leq b$. Further, RM$(m,r)\subset \text{RM}(m,r^\prime)$, for $0\leq r< r^\prime\leq m$, and any codeword ${c}\in \text{RM}(m,r)$ can be written as the concatenation ${c} = \left(u \mid u+v\right)$, where $u\in \text{RM}(m-1,r)$ and $v\in \text{RM}(m-1,r-1)$, for $r\leq m-1$. This hence means that Lemmas \ref{lem:1} and \ref{lem:2} can be employed to compute the weight distributions of RM codes, in a recursive manner, by computing the weight distributions of cosets of one RM code within another.

Now, following \cite{yao}, we show that the weight distributions of certain cosets of RM$(m,r)$ in RM$(m,r^\prime)$, for $r<r^\prime$, are equal. First, let us define the coset
\[
\cC_f:= \text{Eval}(f) + \text{RM}(m,r),
\]
of RM$(m,r)$ in RM$(m,r^\prime)$, where $\text{deg}(f)\leq r^\prime$. %is such that all monomials in its (unique) expansion have their degrees in $[r+1:r^\prime]$. 
Further, for any $p\in \mathbb{F}_2[x_1,\ldots,x_m]$, we define the set $\cM_p:= p+\text{span}(\{g\in \mathbb{F}_2[x_1,\ldots,x_m]:\ \text{deg}(g)\leq r\})$. It is easy to check that all the cosets of RM$(m,r)$ in RM$(m,r^\prime)$ can be written as $\cC_f$ for some $f$, and that the words in $\cC_f$ are evaluations of the polynomials in the set $\cM_f$. Also, it is sufficient to restrict attention to those $\cC_f$ where $f$ is such that all monomials in its (unique) expansion have their degrees in $[r+1:r^\prime]$.

Second, we recall another important property of RM codes, which is the structure of its automorphism group. Recall that if $S_N$ is the symmetric group on $N$ elements, the automorphism group of a length-$N$ code $\cC$ is given by
\[
\text{Aut}(\cC) = \{\pi\in S_N: \pi(c)\in \cC, \text{ for all } c\in \cC\}.
\]
Consider the general affine group GA$(m,2)$ consisting of affine permutations $(A,b)$ of $m$-tuples $y = (y_1,\ldots,y_m)\in \{0,1\}^m$, given by the maps
\[
y \mapsto Ay + b,\ A\in \mathbb{F}_2^{m\times m},\ b\in \mathbb{F}_2^m,
\]
where the matrix $A$ is invertible. It is well-known (see, for example, Theorem 24 in \cite[Chapter 13]{mws}) that Aut$(\text{RM}(m,r)) = \text{GA}(m,2)$, for all $1\leq r\leq m-2$, and Aut$(\text{RM}(m,r))= S_{2^m}\supset \text{GA}(m,2)$, for $r\in \{0,m-1,m\}$. Now, for a polynomial $f \in \mathbb{F}_2[x_1,\ldots,x_m]$, we define $(A,b)\cdot f:= \left(f(Ay+b): y \in \{0,1\}^m\right)$ to be the action of the permutation $(A,b)\in \text{GA}(m,2)$ on $f$. The action of $(A,b)$ on a subset $X\subseteq \mathbb{F}_2[x_1,\ldots,x_m]$, written as $(A,b)\cdot X$, can be defined similarly to be the set of actions of $(A,b)$ on the polynomials in $X$.

Now, observe that for $(A,b)\in \text{GA}(m,2)$, and for $f$ such that deg$(f)\leq r^\prime$, 
\begin{align*}
	(A,b)\cdot \cM_f &= (A,b)\cdot f + \text{span}(\{g:\ \text{deg}(g)\leq r\})\\
	&= h + \text{span}(\{g:\ \text{deg}(g)\leq r\}) = \cM_h,
\end{align*}
for $h = (A,b)\cdot f\in \mathbb{F}_2[x_1,\ldots,x_m]$. Note that the first equality holds since the vector space $\text{span}(\{g:\ \text{deg}(g)\leq r\})$ is invariant under the action of $(A,b)$. It can be argued that deg$(h)\leq r^\prime$, and hence that the evaluations of polynomials in $\cM_h$ give rise to a coset of RM$(m,r)$ in RM$(m,r^\prime)$. Finally, since permutations of coordinates preserve the weights of words, and hence the weight distribution of cosets, it holds that the weight enumerator polynomials $A_{\cC_f}(z)$ and $A_{\cC_h}(z)$, where $h = (A,b)\cdot f$, are equal.
